HEAR: Holistic Evaluation of Audio Representations

What audio embedding approach generalizes best to a wide range of downstream tasks across a variety of everyday domains without fine-tuning? The aim of the HEAR benchmark is to develop a general-purpose audio representation that provides a strong basis for learning in a wide variety of tasks and scenarios. HEAR evaluates audio representations using a benchmark suite across a variety of domains, including speech, environmental sound, and music. HEAR was launched as a NeurIPS 2021 shared challenge. In the spirit of shared exchange, each participant submitted an audio embedding model following a common API that is general-purpose, open-source, and freely available to use. Twenty-nine models by thirteen external teams were evaluated on nineteen diverse downstream tasks derived from sixteen datasets. Open evaluation code, submitted models and datasets are key contributions, enabling comprehensive and reproducible evaluation, as well as previously impossible longitudinal studies. It still remains an open question whether one single general-purpose audio representation can perform as holistically as the human ear.

==> results/model-v-task.tex <==
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllllllllllllllll}
\toprule
task\_with\_primary\_score & \rotatebox{90}{Beehive} & \rotatebox{90}{Beijing Opera} & \rotatebox{90}{CREMA-D} & \rotatebox{90}{DCASE 2016} & \rotatebox{90}{ESC-50} & \rotatebox{90}{FSD50k} & \rotatebox{90}{GTZAN Genre} & \rotatebox{90}{GTZAN Music/Speech} & \rotatebox{90}{Gunshot} & \rotatebox{90}{Libricount} & \rotatebox{90}{Maestro 5h} & \rotatebox{90}{Mridangam Stroke} & \rotatebox{90}{Mridangam Tonic} & \rotatebox{90}{NSynth Pitch 50h} & \rotatebox{90}{NSynth Pitch 5h} & \rotatebox{90}{Speech commands 5h} & \rotatebox{90}{Speech commands full} & \rotatebox{90}{Vocal Imitation} & \rotatebox{90}{VoxLingua107 top 10} \\
model                    &                         &                               &                         &                            &                        &                        &                             &                                    &                         &                            &                            &                                  &                                 &                                  &                                 &                                    &                                      &                                 &                                     \\
\midrule
GURA Fuse Cat H+w+C      &                         &                   {\em 0.966} &             {\em 0.747} &                      0.826 &                  0.734 &                   0.42 &                       0.805 &                              0.928 &                   0.935 &                {\em 0.697} &                      0.441 &                            0.972 &                           0.923 &                            0.885 &                           0.846 &                        {\em 0.961} &                          {\em 0.968} &                     {\em 0.197} &                          {\em 0.72} \\
GURA Fuse Cat H+w+C (t)  &                         &                         0.962 &             {\em 0.743} &                      0.826 &                  0.653 &                  0.374 &                        0.76 &                              0.944 &                   0.905 &                      0.659 &                      0.441 &                      {\em 0.975} &                           0.924 &                            0.891 &                           0.854 &                              0.951 &                          {\em 0.968} &                     {\em 0.215} &                               0.629 \\
GURA Fuse Hubert         &                         &                         0.949 &             {\em 0.752} &                      0.826 &                  0.743 &                  0.413 &                       0.796 &                              0.936 &                   0.929 &                      0.683 &                      0.166 &                      {\em 0.974} &                           0.909 &                            0.688 &                           0.382 &                              0.947 &                                0.957 &                     {\em 0.185} &                         {\em 0.714} \\
GURA Fuse wav2vec2       &                         &                         0.945 &                   0.692 &                      0.798 &                  0.695 &                  0.403 &                       0.793 &                              0.953 &             {\em 0.967} &                      0.653 &                      0.111 &                            0.962 &                           0.838 &                            0.606 &                            0.33 &                        {\em 0.957} &                          {\em 0.969} &                           0.174 &                         {\em 0.706} \\
Logitech SERAB BYOL-S    &                   0.549 &                         0.953 &                   0.657 &                      0.642 &                  0.805 &                  0.509 &                       0.837 &                              0.938 &                   0.857 &                {\em 0.785} &                      0.008 &                      {\em 0.973} &                     {\em 0.928} &                            0.712 &                           0.396 &                              0.914 &                                0.948 &                            0.16 &                               0.458 \\
GURA Cat H+w+C           &                         &                         0.936 &                   0.639 &                      0.681 &                  0.511 &                  0.314 &                       0.722 &                              0.961 &                   0.881 &                      0.639 &                {\em 0.469} &                            0.938 &                           0.859 &                      {\em 0.897} &                           0.866 &                              0.927 &                                0.943 &                           0.111 &                                0.46 \\
CP-JKU PaSST 2lvl+mel    &                         &                   {\em 0.966} &                    0.61 &                {\em 0.925} &            {\em 0.947} &            {\em 0.641} &                 {\em 0.883} &                        {\em 0.977} &                    0.94 &                       0.66 &                            &                            0.965 &                           0.819 &                            0.541 &                           0.256 &                              0.681 &                                0.639 &                           0.182 &                               0.259 \\
CP-JKU PaSST 2lvl        &                         &                   {\em 0.966} &                    0.61 &                {\em 0.913} &            {\em 0.947} &            {\em 0.641} &                 {\em 0.883} &                        {\em 0.977} &                    0.94 &                       0.66 &                            &                            0.965 &                           0.819 &                            0.541 &                           0.256 &                              0.681 &                                0.639 &                           0.182 &                               0.259 \\
CP-JKU PaSST base        &                         &                   {\em 0.966} &                    0.61 &                      0.788 &            {\em 0.947} &            {\em 0.641} &                 {\em 0.883} &                        {\em 0.977} &                    0.94 &                       0.66 &                            &                            0.965 &                           0.819 &                            0.541 &                           0.256 &                              0.681 &                                0.639 &                           0.182 &                               0.259 \\
OpenL3                   &                   0.604 &                   {\em 0.975} &                    0.55 &                {\em 0.833} &                  0.751 &                  0.447 &                       0.879 &                              0.969 &             {\em 0.949} &                      0.641 &                      0.017 &                            0.967 &                     {\em 0.937} &                            0.731 &                            0.56 &                               0.68 &                                0.763 &                           0.078 &                               0.331 \\
GURA Avg H+w+C           &                         &                         0.945 &                   0.547 &                      0.624 &                   0.45 &                  0.264 &                       0.706 &                              0.937 &                   0.857 &                      0.631 &                       0.46 &                            0.914 &                           0.837 &                            0.896 &                           0.862 &                              0.822 &                                0.881 &                           0.084 &                               0.321 \\
GURA Hubert              &                         &                         0.945 &                    0.69 &                      0.584 &                  0.603 &                  0.314 &                       0.735 &                              0.913 &                   0.932 &                      0.646 &                      0.007 &                            0.953 &                            0.85 &                            0.429 &                           0.184 &                              0.953 &                                0.954 &                           0.154 &                               0.637 \\
wav2vec2                 &                         &                         0.907 &                   0.656 &                      0.663 &                  0.561 &                  0.342 &                        0.78 &                              0.946 &                   0.848 &                {\em 0.692} &                      0.033 &                            0.943 &                           0.828 &                            0.653 &                           0.402 &                              0.838 &                                0.879 &                            0.08 &                               0.493 \\
GURA Cat Hubert+wav2vec2 &                         &                         0.936 &                   0.698 &                      0.452 &                  0.586 &                  0.323 &                       0.734 &                              0.936 &                   0.869 &                      0.627 &                      0.003 &                            0.951 &                           0.802 &                            0.428 &                           0.198 &                              0.936 &                                0.929 &                           0.166 &                         {\em 0.706} \\
GURA Avg Hubert+CREPE    &                         &                         0.932 &                    0.54 &                       0.61 &                  0.437 &                  0.253 &                       0.698 &                              0.946 &                   0.845 &                      0.622 &                {\em 0.462} &                            0.917 &                           0.831 &                      {\em 0.897} &                     {\em 0.878} &                              0.737 &                                0.823 &                           0.079 &                               0.293 \\
RedRice EfficientNet-B2  &                   0.533 &                         0.953 &                   0.575 &                       0.79 &                  0.935 &                  0.607 &                       0.878 &                              0.968 &                   0.878 &                      0.651 &                        0.0 &                            0.949 &                           0.843 &                            0.391 &                           0.168 &                              0.573 &                                0.676 &                           0.138 &                               0.255 \\
GURA Avg Hubert+wav2vec2 &                         &                         0.941 &                   0.699 &                      0.417 &                  0.587 &                  0.318 &                       0.746 &                              0.928 &                    0.81 &                      0.623 &                      0.004 &                            0.946 &                           0.799 &                            0.415 &                           0.198 &                              0.907 &                                0.952 &                           0.165 &                                0.69 \\
GURA Cat wav2vec2+CREPE  &                         &                          0.92 &                    0.46 &                      0.585 &                  0.343 &                  0.234 &                       0.681 &                              0.938 &                   0.833 &                      0.569 &                {\em 0.463} &                            0.898 &                           0.823 &                      {\em 0.899} &                     {\em 0.868} &                              0.885 &                                0.919 &                           0.076 &                                0.31 \\
CVSSP PANNS              &                   0.446 &                         0.911 &                   0.555 &                        0.0 &                  0.909 &                        &                        0.86 &                        {\em 0.992} &                   0.798 &                      0.652 &                        0.0 &                            0.939 &                           0.824 &                            0.301 &                           0.148 &                               0.56 &                                0.618 &                           0.127 &                               0.244 \\
IUT-CSE MLP (keyword)    &              {\em 0.76} &                         0.911 &                   0.424 &                      0.518 &                  0.367 &                  0.187 &                       0.554 &                              0.889 &                   0.932 &                      0.451 &                      0.065 &                            0.969 &                     {\em 0.942} &                            0.605 &                            0.44 &                        {\em 0.976} &                          {\em 0.978} &                           0.056 &                               0.181 \\
Sony UDONS ViT           &             {\em 0.878} &                         0.928 &                   0.441 &                      0.668 &                  0.401 &                        &                       0.681 &                              0.899 &                   0.866 &                      0.488 &                      0.239 &                             0.88 &                            0.73 &                            0.795 &                           0.692 &                              0.479 &                                0.531 &                           0.068 &                               0.224 \\
Stellenbosch LSL DBERT   &                   0.697 &                         0.919 &                   0.522 &                      0.246 &                  0.532 &                  0.263 &                       0.674 &                              0.969 &                    0.81 &                      0.584 &                        0.0 &                            0.835 &                           0.685 &                            0.737 &                           0.524 &                              0.566 &                                 0.63 &                           0.161 &                               0.246 \\
Descript/MARL Wav2CLIP   &              {\em 0.77} &                         0.936 &                   0.512 &                        0.0 &                  0.759 &                  0.362 &                       0.748 &                              0.946 &                   0.929 &                      0.528 &                        0.0 &                            0.947 &                           0.829 &                            0.439 &                            0.23 &                              0.316 &                                0.347 &                           0.083 &                               0.192 \\
CREPE                    &                   0.593 &                         0.928 &                   0.383 &                      0.504 &                    0.3 &                  0.159 &                       0.645 &                              0.929 &                   0.863 &                      0.499 &                      0.401 &                            0.898 &                           0.824 &                        {\em 0.9} &                      {\em 0.87} &                               0.18 &                                0.211 &                           0.051 &                               0.142 \\
Soundsensing YAMNet      &                   0.466 &                         0.941 &                   0.453 &                      0.008 &                  0.838 &                        &                       0.847 &                              0.969 &                   0.732 &                      0.653 &                        0.0 &                                  &                                 &                            0.321 &                           0.158 &                              0.289 &                                 0.41 &                           0.085 &                               0.202 \\
Kuroyanagi hearline      &                         &                         0.928 &                    0.48 &                            &                  0.424 &                  0.178 &                       0.654 &                              0.931 &                   0.518 &                      0.498 &                      0.002 &                            0.909 &                           0.783 &                            0.589 &                           0.394 &                              0.478 &                                 0.58 &                            0.04 &                                0.18 \\
AMAAI w2v2 music+spch    &                         &                         0.826 &                   0.391 &                       0.51 &                  0.511 &                  0.198 &                       0.605 &                              0.907 &                   0.857 &                      0.432 &                      0.003 &                            0.759 &                           0.415 &                            0.176 &                           0.182 &                              0.744 &                                0.523 &                           0.064 &                               0.169 \\
IUT-CSE MLP (audio)      &                   0.535 &                         0.728 &                    0.42 &                      0.052 &                  0.161 &                  0.086 &                       0.408 &                              0.774 &                   0.786 &                      0.366 &                      0.024 &                            0.893 &                           0.778 &                            0.608 &                           0.386 &                              0.392 &                                0.535 &                           0.038 &                               0.129 \\
AMAAI Lab w2v2+DDSP      &                         &                         0.635 &                         &                      0.507 &                   0.28 &                  0.268 &                             &                                    &                   0.583 &                       0.51 &                        0.0 &                            0.653 &                           0.357 &                            0.303 &                           0.172 &                              0.487 &                                 0.49 &                           0.072 &                               0.106 \\
\bottomrule
\end{tabular}

}
